Empirical likelihood test for community structure in networks

Network data, characterized by interconnected nodes and edges, is pervasive in various domains and has gained significant popularity in recent years. In network data analysis, testing the presence of community structure in a network is one of the important research tasks. Existing tests are mainly developed for unweighted networks. In this paper, we study the problem of testing the existence of community structure in general (either weighted or unweighted) networks. We propose two new tests: the Weighted Signed-Triangle (WST) test and the empirical likelihood (EL) test. Both tests can be applied to weighted or unweighted networks and outperform existing tests for small networks. The EL test may outperform the WST test for small networks.

==> marco.tex <==
\newcommand{\ind}[1]{\1_{\{ #1\}}}
\newcommand{\borel}{\mathscr{B}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\law}{\mathfrak{L}}
\newcommand{\ct}[1]{\stackrel{#1}{\longrightarrow}}

\newtheorem{exmp}{Example}[section]
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

\usepackage{amsmath}
\usepackage{amssymb}%花体字母加粗
\usepackage{mathrsfs}%花体字母
\usepackage[flushleft]{threeparttable}
\usepackage{enumitem}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%date
%\def\headline {{\rm \number\month-\number\day-\number\year}\hfill
%               \par\vskip 15pt}
%\def\today{\ifcase\month\or
% January\or February\or March\or April\or May\or June\or
% July\or August\or September\or October\or November\or December\fi
% \space\number\day, \number\year}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%
\def\bDef{\begin{definition}}
\def\eDef{\end{definition}}
\def\bThm{\begin{theorem}}
\def\eThm{\end{theorem}}
\def\bCor{\begin{corollary}}
\def\eCor{\end{corollary}}
\def\bProp{\begin{proposition}}
\def\eProp{\end{proposition}}
\def\bLm{\begin{lemma}}
\def\eLm{\end{lemma}}
\def\bEx{\begin{example}}
\def\eEx{\end{example}}
\def\bRem{\begin{remark}}
\def\eRem{\end{remark}}
\def\bPf{\begin{proof}}
\def\ePf{\end{proof}}
\def\bAssump{\begin{assumption}}
\def\eAssump{\end{assumption}}


%%%%%%%%%%%%%%%%%
\numberwithin{equation}{section}
%\theoremstyle{plain}
\def\varnothing{\mathchoice{\mbox{\msbmx\char'077}}%
{\mbox{\msbmx\char'077}}{\mbox{\msbmvii\char'077}}{\mbox{\msbmv\char'077}}}%
\def\Cov{\mathop{\rm Cov}\nolimits}% % A sample of proper declaration of
\def\Argmax{\mathop{\arg\max}\limits}%    a math operator.
\def\Var{\mathop{\mathrm{Var}}\nolimits}%
\def\R{\mathbb R}
\def\x{\times}
\def\vt{\vartheta}
\def\ve{\varepsilon}
\def\el{\mathscr{R}_{n}}
\def\elcs{\mathscr{R}_{n}^{cs}}

\def\prob{\mathcal{P}_{n}}
\def\und{\quad \mbox{and} \quad}
\def\where{\quad \mbox{where} \quad}
\def\1{\mathbf 1}
\def\ave{\frac{1}{n}\sum_{j=1}^n}
\def\Ave{\frac{1}{n}\sum_{j=1}^n}
\def\pave{\sum_{j=1}^n \pi_j}
\def\maxj{\max_{1\leq j \leq n}}
\def\minj{\min_{1\leq j \leq n}}
\def\hz{\hat\zeta_n}
\def\vG{\varGamma_n}
\def\trace{\mathrm{trace}}
\def\sign{\mathrm{sign}}
\def\sQ{{\mathscr Q}}
\def\sZ{{\mathcal Z}}
\def\zt{\zeta}
\def\sV{\mathscr{V}}
\def\cA{\mathcal A}
\def\bS{\mathbb S}
\def\T{\mathbb T}
\def\vt{\vartheta}
\def\hvt{\hat\theta}
\def\tvt{\tilde\theta}
\def\ql{Qin and Lawless (1994)~}
\def\hmk{Hjort et al (2009)~}
\def\msw{M\"uller et al~}
\def \save{n^{-1/2}\sum_{j=1}^n}
\def\ve{\varepsilon}
\def\he{\hat \varepsilon}
\def\emp{\mathbb{F}}
\def\hemp{\hat\emp}
\def\hRone{\mathscr{R}_{n1}}
\def\hRtwo{\mathscr{R}_{n2}}
\newcommand{\hhR}[1]{\hat{\mathscr{R}}_{#1}}
\def\hF{\hat{\hat F}_n}
\newcommand{\sel}[1]{\sup\Big\{ \prod_{j=1}^n n\pi_j: \pi\in \prob, #1
\Big\}}
\newcommand{\ssel}[1]{\sup\Big\{ \prod_{j=1}^n n\pi_j: &
(\pi_1,\dots,\pi_n)\in \Pi_n, \\ & #1 \Big\}}
\def\gchi{\mathscr{G}}
\def\LL{\mathscr{L}_n}
\def\hLL{\hat{\mathscr{L}}_{n}}
%\def\z{\mathfrak{z}}
\def\ldot{\dot \ell}
%\def\gemp{\mathbb{G}_n}
\def\femp{\mathbb{F}_n}
\def\sfemp{\tilde {\mathbb{F}}_n}
\def\opti{central~}
\def\opte{central}
\def\op{o_P(1)}
\def\opn{o_P(n^{-1/2})}
\def\tM{\tilde M}
%\def\kQ{\kappa(Q)}
\def\kQ{\theta}

\def\bu{\bar{U}_{n}}
\def\tu{\tilde{U}_{n}}
\def\hu{\hat{U}_{n}}
\def\hR{{\hat R}}
\def\hb{{\hat b}}
\def\sbtheta{{\bdm{\hat\theta}^*}}


\def\Unif{\mathrm{Unif}}
\def\MSE{{\mathrm{MSE}}}

\def\L{\mathrm{L}}
\def\b{\mathbf{b}}
\def\u{\mathbf{u}}
\def\jsum{\sum_{j=1}^n}
\def\lksum{\sum_{l=0}^{k-1}}
\def\htet{\hat\theta} 
\def\seq#1{\{#1\}}
\def\sq#1{\left\{#1\right\}}

\def\ps{Peng and Schick (2011)} 
\def\jave{\frac{1}{n}\sum_{j=1}^n}
\def\iave{\frac{1}{n}\sum_{i=1}^n}

\def\diag{\textrm{diag}}
\def\tr{\mathrm{Tr}}
\def\lam{\lambda}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\seq#1{\left\{#1\right\}}
\def\PS{Peng and Schick}
\def\jave{\frac{1}{n}\sum_{j=1}^n}
\def\BKRW{\textrm{Bickel, Klasseen, Ritov and Wellner (1993)}}
\def\hR{{\hat R}}
\def\jprod{\prod_{j=1}^n}

\def\AVar{\mathrm{AVar}}


%%%%%%%%%%%
\def\hB{{\hat B}}
\def\bhb{{\bar{\hat b}}_n}
\def\Bin{\textrm{Bin}}
\def\deq {\overset{d}{=}}
\def\pconv{\overset{p}{\longrightarrow}}


\def\sgn{\textrm{sgn}}
\def\hmu{\hat\mu_n}
\def\tmu{\tilde\mu_n}
\def\SU{\mathbb U}

\def\rE{\rm{E}}
\def\rV{\rm{Var}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bA{{\mathbb{A}}}
\def\bB{{\mathbb{B}}}
\def\bC{{\mathbb{C}}}
\def\bD{{\mathbb{D}}}
\def\bE{{\mathbb{E}}}
\def\bF{{\mathbb{F}}}
\def\bG{{\mathbb{G}}}
\def\bH{{\mathbb{H}}}
\def\bI{{\mathbb{I}}}
\def\bJ{{\mathbb{J}}}
\def\bK{{\mathbb{K}}}
\def\bL{{\mathbb{L}}}
\def\bM{{\mathbb{M}}}
\def\bN{{\mathbb{N}}}
\def\bO{{\mathbb{O}}}
\def\bP{{\mathbb{P}}}
\def\bQ{{\mathbb{Q}}}
\def\bR{{\mathbb{R}}}
\def\bS{{\mathbb{S}}}
\def\bT{{\mathbb{T}}}
\def\bU{{\mathbb{U}}}
\def\bV{{\mathbb{V}}}
\def\bW{{\mathbb{W}}}
\def\bX{{\mathbb{X}}}
\def\bY{{\mathbb{Y}}}
\def\bZ{{\mathbb{Z}}}



\def\sA{{\mathscr{A}}}
\def\sB{{\mathscr{B}}}
\def\sC{{\mathscr{C}}}
\def\sD{{\mathscr{D}}}
\def\sE{{\mathscr{E}}}
\def\sF{{\mathscr{F}}}
\def\sG{{\mathscr{G}}}
\def\sH{{\mathscr{H}}}
\def\sI{{\mathscr{I}}}
\def\sJ{{\mathscr{J}}}
\def\sK{{\mathscr{K}}}
\def\sL{{\mathscr{L}}}
\def\sM{{\mathscr{M}}}
\def\sN{{\mathscr{N}}}
\def\sO{{\mathscr{O}}}
\def\sP{{\mathscr{P}}}
\def\sQ{{\mathscr{Q}}}
\def\sR{{\mathscr{R}}}
\def\sS{{\mathscr{S}}}
\def\sT{{\mathscr{T}}}
\def\sU{{\mathscr{U}}}
\def\sV{{\mathscr{V}}}
\def\sW{{\mathscr{W}}}
\def\sX{{\mathscr{X}}}
\def\sY{{\mathscr{Y}}}
\def\sZ{{\mathscr{Z}}}

\def\rP{{\mathrm{P}}}


\def\A{{\mathbf{A}}}
\def\B{{\mathbf{B}}}
\def\C{{\mathbf{C}}}
\def\D{{\mathbf{D}}}
\def\E{{\mathbf{E}}}
\def\F{{\mathbf{F}}}
\def\G{{\mathbf{G}}}
\def\H{{\mathbf{H}}}
\def\I{{\mathbf{I}}}
\def\J{{\mathbf{J}}}
\def\K{{\mathbf{K}}}
\def\L{{\mathbf{L}}}
\def\M{{\mathbf{M}}}
\def\N{{\mathbf{N}}}
\def\O{{\mathbf{O}}}
\def\P{{\mathbf{P}}}
\def\mQ{{\mathbf{Q}}}
\def\R{{\mathbf{R}}}
\def\S{{\mathbf{S}}}
\def\T{{\mathbf{T}}}
\def\U{{\mathbf{U}}}
\def\V{{\mathbf{V}}}
\def\W{{\mathbf{W}}}
\def\X{{\mathbf{X}}}
\def\Y{{\mathbf{Y}}}
\def\mZ{{\mathbf{Z}}}
\def\mA{{\mathbf{A}}}
\def\mH{{\mathbf{H}}}
\def\mB{{\mathbf{B}}}
\def\tdmH{\tilde{\mathbf{H}}}
\def\th{\tilde{h}}


\def\a{{\bm{a}}}
\def\b{{\bm{b}}}
\def\c{{\bm{c}}}
\def\d{{\bm{d}}}
\def\e{{\bm{e}}}
\def\f{{\bm{f}}}
\def\g{{\bm{g}}}
\def\h{{\bm{h}}}
\def\i{{\bm{i}}}
\def\j{{\bm{j}}}
\def\k{{\bm{k}}}
\def\l{{\bm{l}}}
\def\m{{\bm{m}}}
\def\n{{\bm{n}}}
\def\o{{\bm{o}}}
\def\p{{\bm{p}}}
\def\q{{\bm{q}}}
\def\r{{\bm{r}}}
\def\s{{\bm{s}}}
\def\t{{\bm{t}}}
\def\u{{\bm{u}}}
\def\v{{\bm{v}}}
\def\w{{\bm{w}}}
\def\x{{\bm{x}}}
\def\y{{\bm{y}}}
\def\z{{\bm{z}}}

\def\cA{{\mathcal{A}}}
\def\cB{{\mathcal{B}}}
\def\cC{{\mathcal{C}}}
\def\cD{{\mathcal{D}}}
\def\cE{{\mathcal{E}}}
\def\cF{{\mathcal{F}}}
\def\cG{{\mathcal{G}}}
\def\cH{{\mathcal{H}}}
\def\cI{{\mathcal{I}}}
\def\cJ{{\mathcal{J}}}
\def\cK{{\mathcal{K}}}
\def\cL{{\mathcal{L}}}
\def\cM{{\mathcal{M}}}
\def\cN{{\mathcal{N}}} 
\def\cO{{\mathcal{O}}}
\def\cP{{\mathcal{P}}}
\def\cQ{{\mathcal{Q}}}
\def\cR{{\mathcal{R}}}
\def\cS{{\mathcal{S}}}
\def\cT{{\mathcal{T}}}
\def\cU{{\mathcal{U}}}
\def\cV{{\mathcal{V}}}
\def\cW{{\mathcal{W}}}
\def\cX{{\mathcal{X}}}
\def\cY{{\mathcal{Y}}}
\def\cZ{{\mathcal{Z}}}

\def\cTheta{{\mathcal{\Theta}}}


\def\bfV{{\boldface{V}}}



\def\bdm#1{\mbox{\boldmath$#1$\unboldmath}}
\def\balpha{\bdm{\alpha}}
\def\bbeta{\bdm{\beta}}
\def\bgamma{{\bdm{\gamma}}}
\def\bdelta{\bdm{\delta}}
\def\bepsilon{\bdm{\epsilon}}
\def\ep{\epsilon}
\def\bep{\bdm{\epsilon}}
\def\bvep{\bdm{\varepsilon}}
\def\vep{\varepsilon}
\def\bvep{\bdm{\varepsilon}}
\def\bzeta{\bdm{\zeta}}
\def\ceta{\bdm{\eta}}
\def\btheta{\bdm{\theta}}
\def\bkappa{\bdm{\kappa}}
\def\blambda{\bdm{\lambda}}
\def\bmu{\bdm{\mu}}
\def\bnu{\bdm{\nu}}
\def\bksi{\bdm{\ksi}}
\def\bxi{\bdm{\xi}}
\def\ceta{\bdm{\eta}}


\def\bomicron{\bdm{\omicron}}
\def\bpi{\bdm{\pi}}
\def\brho{\bdm{\rho}}
\def\bsigma{\bdm{\sigma}}
\def\btau{\bdm{\tau}}
\def\bupsilon{\bdm{\upsilon}}
\def\bphi{\bdm{\phi}}
%\def\bvarphi{\bdm{\varphi}}}
\def\bchi{\bdm{\chi}}
\def\bpsi{\bdm{\psi}}
%\def\bvarpsi{\bdm{\varpsi}}}
\def\bomega{\bdm{\omega}}
\def\Diag{\mathbb D{\mathrm{iag}}}

\def\bAlpha{{\bdm{\Alpha}}}
\def\bBeta{{\bdm{\Beta}}}
\def\bGamma{{\bdm{\Gamma}}}
\def\bDelta{{\bdm{\Delta}}}
\def\bEpsilon{{\bdm{\Epsilon}}}
\def\bZeta{{\bdm{\Zeta}}}
\def\bEta{{\bdm{\Eta}}}
\def\bTheta{{\bdm{\Theta}}}
\def\bKappa{{\bdm{\Kappa}}}
\def\bLambda{{\bdm{\Lambda}}}
\def\bMu{{\bdm{\Mu}}}
\def\bNu{{\bdm{\Nu}}}
\def\bKsi{{\bdm{\Ksi}}}
\def\bOmicron{{\bdm{\Omicron}}}
\def\bPi{{\bdm{\Pi}}}
\def\bRho{{\bdm{\Rho}}}
\def\bSigma{{\bdm{\Sigma}}}
\def\bTau{{\bdm{\Tau}}}
\def\bUpsilon{{\bdm{\Upsilon}}}
\def\bPhi{{\bdm{\Phi}}}
\def\bChi{{\bdm{\Chi}}}
\def\bPsi{{\bdm{\Psi}}}
\def\bOmega{{\bdm{\Omega}}}
\def\ind{{\mathrm{ind}}}
\def\as{{\mathrm{a.s.}}}
\def\say{{\mathrm{say}}}

\def\vs{{\otimes 2}}
\def\hpit{{{\hat\pi^{(l_n)}}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tbtheta{{\hat\btheta^*}}
\def\betolsf{\hat\bbeta_{\mathrm{ols},1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tmat#1#2#3#4#5#6#7#8#9{\left(
\begin{array}{ccc}
{#1} & {#2} & {#3} \\
{#4} & {#5} & {#6} \\
{#7} & {#8} & {#9} 
\end{array}\right)}  


\def\pfun#1#2#3#4{{\left\{
\begin{array}{ll}
{#1} & {#2}  \\
{#3} & {#4} 
\end{array}\right.}} 



\def\smat#1#2#3#4{\left(
\begin{array}{cc}
{#1} & {#2}  \\
{#3} & {#4} 
\end{array}\right)}  

\def\cmat#1#2{\left(
\begin{array}{cc}
{#1} \\
{#2}
\end{array}\right)}

\def\cmatt#1#2#3{\left(
\begin{array}{ccc}
{#1} \\
{#2} \\
{#3}
\end{array}\right)}


\def\ksum{\sum_{k=1}^N}
\def\jrsum{\sum_{j=1}^r}



\def\bea{$$\begin{aligned}}
\def\eea{\end{aligned}$$}

\def\Uj{\U_{n-1}^{(-j)}}
\def\PS12{Peng and Schick (2012)} 
\def\seq#1{\left\{#1\right\}}
\def\pare#1{\left(#1\right)}
\def\squ#1{\left[#1\right]}
\def\uave{{n \choose m}^{-1} \sum_{1\leq i_1<\ldots<i_m\leq n}}
\def\pU{\U^\#}
\def\PL{PL (2013)}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tbeta{{\tilde\beta}}
\def\tbbeta{{\hat\bbeta_{r}^*}}

\def\tbeta{{\beta^*}}
%\def\bDiag{{\textrm{Diag}}}
\def\etal {{\sl et al.}}

\def\Diag{{\textrm{Diag}}}
\def\Vec{{\textrm{Vec}}}

%\def\betols{\hat{\bdm{\bbeta}}_{\mathrm{lse}}}
%\def\hbbeta{\hat{\bdm{\beta}}_{\mathrm{ols}}}


\def\bCov{{\mathbb{C}\mathrm{ov}}}
\def\bVar{{\mathrm{V}\mathrm{ar}}}
\def\rCov{{\mathrm{C}\mathrm{ov}}}
\def\rVar{{\mathrm{V}\mathrm{ar}}}
\def\rE{{\mathrm{E}}}
\def\rP{{\mathrm{P}}}
\def\rF{{\mathrm{F}}}

\def\bDiag{{\mathrm{D}\mathrm{iag}}}
\def\rDiag{{\mathrm{D}\mathrm{iag}}}
\def\bTr{{\mathrm{T}\mathrm{r}}}
\def\rTr{{\mathrm{T}\mathrm{r}}}
\def\Normal{{\mathcal{N}}}
\def\ahpi{{\hat\pi^{(2\alpha)}}}
\def\ARE{{\mathbb{ARE}}}
\def\unif{{\textrm{UNIF}}}

\def\hbpi{{\hat{\bpi}_{\mathrm{aopt}}}}
\def\bbpi{{\bar{\bpi}_{\mathrm{aopt}}}}
\def\tbpi{{\tilde{\bpi}_{\mathrm{aopt}}}}


\def\hpi{{\hat{\pi}}}
\def\bbpi{{\bar{\pi}}}


\def\barbpi{{\bar{\bpi}_{\mathrm{aopt}}}}
\def\barpi{{\bar{\pi}^{\mathrm{(aopt)}}}}

\def\tbpi{{\tilde{\bpi}_{\mathrm{aopt}}}}
\def\tpi{{\tilde{\pi}^{\mathrm{(aopt)}}}}

\def\aopt{{\mathrm{aopt}}}

\def\UNIF{{\mathrm{UNIF}}}
%%%%%%%%%%%%%%%%%%%
\def\h1#1{{h_{#1}^{(1)}}}
\def\ejlt{{$\epsilon$-JLT}}
\def\ejlts{{$\epsilon_2$-JLT}}
\def\fejlt{{$\epsilon$-FJLT}}
\def\fejltf{{$\epsilon_1$-FJLT}}
\def\Mult{{\mathrm{Mult}}}
\def\sMult{{\mathrm{sMult}}}
\def\Bias{\mathrm{Bias}}
\def\Deltad{\bigtriangledown}
\def\inprob{{in\ probability}}
\def\pas{{P\ a.s.}}

%%%%%%%%%%%%%%%%%%
\def\CB{Chatterjee and Bose (2005)}
\def\hbeta{{\hat\beta_n}}

\def\sbeta{{\hat\beta_{r_n}^*}}
\def\sbetaz{{\hat\beta_{r_n,0}^*}}
\def\hpsi{{\hat\psi}}
\def\amin{{\mathrm{amin}}}
\def\amax{{\mathrm{amax}}}

\def\tdX{{\tilde{\X}}}
\def\tdx{{\tilde{\x}}}
\def\tde{{\tilde{\e}}}
\def\tdvep{{\tilde{\varepsilon}}}
\def\tdH{{\tilde{\mH}}}
\def\tdh{{\tilde{\h}}}

%%%


